A Faster Algorithm for Asymptotic Communication for Omniscience

We propose a modified decomposition algorithm (MDA) to solve the asymptotic communication for omniscience (CO) problem where the communication rates could be real or fractional. By starting with a lower estimation of the minimum sum-rate, the MDA algorithm iteratively updates the estimation by the optimizer of a Dilworth truncation problem until the minimum is reached with a corresponding optimal rate vector. We also propose a fusion method implementation of the coordinate-wise saturation capacity algorithm (CoordSatCapFus) for solving the Dilworth truncation problem, where the minimization is done over a fused user set with a cardinality smaller than the original one. We show that the MDA algorithm is less complex than the existing ones. In addition, we show that the non-asymptotic CO problem, where the communication rates are integral, can be solved by one more call of the CoordSatCapfus algorithm. By choosing a proper linear ordering of the user indices in the MDA algorithm, the optimal rate vector is also the one with the minimum weighted sum-rate.

==> figures/PLPdemo.tex <==
% This file was created by matlab2tikz v0.4.3.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
%
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[
every pin edge/.style={<-}]

\begin{axis}[%
width=4in,
height=2.8in,
scale only axis,
xmin=0,
xmax=11,
xlabel={\Large $\lambda$},
xtick={0,1,2,3,4,5,6,7,8,9,10,11},
xmajorgrids,
ymin=-10,
ymax=11,
ylabel={\Large $L(\lambda)$},
ymajorgrids
]
\addplot [
color=blue,
solid,
line width=2.0pt,
mark=o,
mark options={solid},
forget plot
]
table[row sep=crcr]{
0 8\\
2 6\\
3 4\\
5 -2\\
11 -26\\
};

% critical points
\node at (axis cs:0,8) [pin={20:\textcolor{red}{$\lambda_0=0,\Pat_0^-=\Set{V}$}}] {};
\node at (axis cs:2,6) [pin={30:\textcolor{red}{$\lambda_1=2,\Pat_1^-=\Set{\Set{1,2,3},\Set{4}}$}}] {};
\node at (axis cs:3,4) [pin={30:\textcolor{red}{$\lambda_2=3,\Pat_2^-=\Set{\Set{1,3},\Set{2},\Set{4}}$}}] {};
\node at (axis cs:5,-2) [pin={80:\textcolor{red}{$\lambda_3=5,\Pat_3^-=\Set{\Set{1},\Set{2},\Set{3},\Set{4}}$}}] {};

% gradient
\node at (axis cs:0.7,7.2) [pin={-90:\textcolor{green}{$d_1=-1$}}] {};
\node at (axis cs:2.5,5) [pin={-100:\textcolor{green}{$d_2=-2$}}] {};
\node at (axis cs:4,1) [pin={-120:\textcolor{green}{$d_3=-3$}}] {};
\node at (axis cs:6,-6) [pin={-120:\textcolor{green}{$d_3=-4$}}] {};

% critical points
\node[pin=20:\textcolor{red}{$\lambda_0=0,\Pat_0=\Set{V}$}] at (0,8) {};
\node[pin=30:\textcolor{red}{$\lambda_1=2,\Pat_1=\Set{\Set{1,2,3},\Set{4}}$}] at (2,6) {};
\node[pin=30:\textcolor{red}{$\lambda_2=3,\Pat_2=\Set{\Set{1,3},\Set{2},\Set{4}}$}] at (3,4) {};
\node[pin=80:\textcolor{red}{$\lambda_3=5,\Pat_3=\Set{\Set{1},\Set{2},\Set{3},\Set{4}}$}] at (5,-2) {};

% gradient
\node[pin=-90:\textcolor{green}{$d_1=-1$}] at (0.7,7.2) {};
\node[pin=-100:\textcolor{green}{$d_2=-2$}] at (2.5,5) {};
\node[pin=-120:\textcolor{green}{$d_3=-3$}] at (4,1) {};
\node[pin=-120:\textcolor{green}{$d_3=-4$}] at (6,-6) {};

\end{axis}
\end{tikzpicture}%

